A portable platform for accelerated PIC codes and its application to GPUs using OpenACC

We present a portable platform, called PIC_ENGINE, for accelerating Particle-In-Cell (PIC) codes on heterogeneous many-core architectures such as Graphic Processing Units (GPUs). The aim of this development is efficient simulations on future exascale systems by allowing different parallelization strategies depending on the application problem and the specific architecture. To this end, this platform contains the basic steps of the PIC algorithm and has been designed as a test bed for different algorithmic options and data structures. Among the architectures that this engine can explore, particular attention is given here to systems equipped with GPUs. The study demonstrates that our portable PIC implementation based on the OpenACC programming model can achieve performance closely matching theoretical predictions. Using the Cray XC30 system, Piz Daint, at the Swiss National Supercomputing Centre (CSCS), we show that PIC_ENGINE running on an NVIDIA Kepler K20X GPU can outperform the one on an Intel Sandybridge 8-core CPU by a factor of 3.4.

==> bibmain.tex <==
%%
%% WinShell 3.3.2.6
%% http://www.winshell.org/
%%

% Strings


% Preamble


% BibTeX Entries

@article{decyk_singh:2014,
  title={Particle-in-Cell algorithms for emerging computer architectures},
  author={Decyk, Viktor K. and Singh, Tajendra V.},
  journal={Comput. Phys. Commun.},
  volume={185},
  number={3},
  pages={708--719},
  year={2014},
  publisher={Elsevier}
}

@article{burnetas_etal:1997,
       author    = {Apostolos Burnetas and Daniel Solow and Rishi Agarwal},
       title     = {An Analysis and Implementation of an Efficient In-Place Bucket Sort},
       year      = {1997},
       journal   = {Acta Informatica},
       volume    = {34},
       pages     = {687--700}}
       
       
@article{jocksch2015bucket,
  title={A bucket sort algorithm for the particle-in-cell method on manycore architectures},
  author={Jocksch, A and Hariri, F and Tran, Track M and Brunner, S and Gheller, C and Villard, L},
  journal={Lecture Notes in Computer Science},
  year={2015},
  publisher={Springer}
}

@article{rozen2008gpu,
  title={GPU bucket sort algorithm with applications to nearest-neighbour search},
  author={Ro{\'z}en, T and Boryczko, Krzysztof and Alda, Witold},
  year={2008},
  publisher={V{\'a}clav Skala-UNION Agency}
}

@article{mertmann_etal:2011,
       author    = {Philipp Mertmann and Denis Eremin and Thomas Mussenbrock and Ralf Peter Brinkmann and Peter Awakowicz},
       title     = {Fine-sorting One-Dimensional Particle-in-Cell Algorithm with {M}onte-{C}arlo Collisions on a Graphics Processing Unit},
       year      = {2011},
       journal   = {Comput. Phys. Commun.},
       volume    = {182},
       pages     = {2161--2167}}

@article{bruck_etal:1997,
       author    = {Jehoshua Bruck and Ching-Tien Ho and Shlomo Kipnis and Eli Upfal and Derrick Weathersby},
       title     = {Efficient Algorithms for All-to-All Communications in Multiport Message-Passing Systems},
       year      = {1997},
       journal   = {IEEE T. Parall. Distr.},
       volume    = {8},
       number    = {11},
       pages     = {1143--1156}}

@article{stantchev_dorland_gumerov:2008,
       author    = {George Stantchev and William Dorland and Nail Gumerov},
       title     = {Fast Parallel {P}article-{T}o-{G}rid Interpolation for Plasma {PIC} Simulations on the {GPU}},
       year      = {2008},
       journal   = {J. Parallel Distrib. Comput.},
       volume    = {68},
       pages     = {1339--1349}}

@article{sintorn_assarsson:2008,
       author    = {Erik Sintorn and Ulf Assarsson},
       title     = {Fast Parallel {GPU}-sorting Using a Hybrid Algorithm},
       year      = {2008},
       journal   = {J. Parallel Distrib. Comput.},
       volume    = {68},
       pages     = {1381--1388}}

@article{maduri_etal:2011,
       author    = {Kamesh Madduri and Eun-Jin Im and Khaled Z. Ibrahim and Samuel Williams and St\'ephane Ethier and Leonid Oliker},
       title     = {Gyrokinetic Particle-in-Cell Optimization on Emerging Multi- and Manycore Platforms},
       year      = {2011},
       journal   = {Parallel Comput.},
       volume    = {37},
       pages     = {501--520}}

@article{chen_chacon_barnes:2012,
       author    = {G. Chen and L. Cha\'con and D.C. Barnes},
       title     = {An Efficient Mixed-Precision, Hybrid {CPU}-{GPU} implementation of a Nonlinearly Implicit One-Dimensional Particle-in-Cell Algorithm},
       year      = {2012},
       journal   = {J. Comput. Phys.},
       volume    = {231},
       pages     = {5374--5388}}

@article{merrill_grimshaw:2011,
       author    = {Duane Merrill and Andrew Grimshaw},
       title     = {High Performance and Scalable Radix Sorting: {A} Case Study of Implementing Dynamic Parallelism for {GPU} Computing},
       year      = {2011},
       journal   = {Parallel Processing Letters},
       volume    = {21},
       number    = {2},
       pages     = {245--272}}

@book{hockney_eastwood:1988,
       author    = {R.W. Hockney and J.W. Eastwood},
       title     = {Computer Simulation Using Particles},
       year      = {1988},
       publisher = {Hilger},
       address   = {Bristol}}
}

@book{TEMPL1994,
author = {Barrett, R. and Berry, M. and Chan, T. and Demmel, J. and Donato, J. and Dongarra, J. and Eijkhout, V. and Pozo, R. and Romine, C. and van der Vorst, H.},
title = {Templates for the Solution of Linear Systems: Building Blocks for Iterative Methods},
publisher = {Society for Industrial and Applied Mathematics},
year = {1994},
doi = {10.1137/1.9781611971538},
address = {},
edition   = {},
URL = {http://epubs.siam.org/doi/abs/10.1137/1.9781611971538},
eprint = {http://epubs.siam.org/doi/pdf/10.1137/1.9781611971538}
}

@book{de2001practical,
  title={A Practical Guide to Splines},
  author={de Boor, C.},
  isbn={9780387953663},
  lccn={20049644},
  series={Applied Mathematical Sciences},
  url={http://books.google.ch/books?id=m0QDJvBI\_ecC},
  year={2001},
  publisher={Springer New York}
}

@inproceedings{joseph_etal:2011,
       author       = {Rejith George Joseph and Girish Ravunnitkutty and Sanjay Ranka and Eduardo D'Azevedo and Scott Klasky},
       title        = {Efficient {GPU} Implementation for Particle in Cell algorithm},
       booktitle    = {25th IEEE International Parallel \& Distributed Processing Symposium (IPDPS)},
       year         = {2011},
       address      = {Anchorage (Alaska)},
       month        = {May}}

@inproceedings{satish_etal:2010,
       author       = {Nadathur Satish and Changkyu Kim and Jatin Chhugani and Anthony D. Nguyen and Viktor W. Lee and Daehyun Kim and Pradeep Dubey},
       title        = {Fast Sort on {CPU}s and {GPU}s: A case for Bandwidth Oblivious {SIMD} Sort},
       booktitle    = {SIGMOD'10},
       year         = {2010},
       address      = {Indinapolis (Indiana)},
       month        = {June}}

@misc{openacc,
   title = {The {O}pen{ACC} standard: www.openacc-standard.org}
}

@misc{cuda,
   title = {The {CUDA} programming model: developer.nvidia.com/cuda-zone}
}

@book{birdsall2004plasma,
  title={Plasma physics via computer simulation},
  author={Birdsall, Charles K and Langdon, A Bruce},
  year={2004},
  publisher={CRC Press}
}

@book{hockney1988computer,
  title={Computer simulation using particles},
  author={Hockney, Roger W and Eastwood, James W},
  year={1988},
  publisher={CRC Press}
}

@article{villard2013global,
  title={Global gyrokinetic ion temperature gradient turbulence simulations of ITER},
  author={Villard, Laurent and Angelino, Paolo and Bottino, Alberto and Brunner, Stephan and Jolliet, S{\'e}bastien and McMillan, BF and Tran, Trach-Minh and Vernay, Thibaut},
  journal={Plasma Physics and Controlled Fusion},
  volume={55},
  number={7},
  pages={074017},
  year={2013},
  publisher={IOP Publishing}
}

@article{bowers2001accelerating,
  title={Accelerating a particle-in-cell simulation using a hybrid counting sort},
  author={Bowers, KJ},
  journal={Journal of Computational Physics},
  volume={173},
  number={2},
  pages={393--411},
  year={2001},
  publisher={Elsevier}
}

@article{tskhakaya2007optimization,
  title={Optimization of PIC codes by improved memory management},
  author={Tskhakaya, David and Schneider, Ralf},
  journal={Journal of Computational Physics},
  volume={225},
  number={1},
  pages={829--839},
  year={2007},
  publisher={Elsevier}
}

@article{decyk1995skeleton,
  title={Skeleton PIC codes for parallel computers},
  author={Decyk, Viktor K},
  journal={Computer Physics Communications},
  volume={87},
  number={1},
  pages={87--94},
  year={1995},
  publisher={Elsevier}
}

@article{stantchev2008fast,
  title={Fast parallel Particle-To-Grid interpolation for plasma PIC simulations on the GPU},
  author={Stantchev, George and Dorland, William and Gumerov, Nail},
  journal={Journal of Parallel and Distributed Computing},
  volume={68},
  number={10},
  pages={1339--1349},
  year={2008},
  publisher={Elsevier}
}

@article{liewer1989general,
  title={A general concurrent algorithm for plasma particle-in-cell simulation codes},
  author={Liewer, Paulett C and Decyk, Viktor K},
  journal={Journal of Computational Physics},
  volume={85},
  number={2},
  pages={302--322},
  year={1989},
  publisher={Elsevier}
}

@article{burau2010picongpu,
  title={PIConGPU: A fully relativistic particle-in-cell code for a GPU cluster},
  author={Burau, Heiko and Widera, Ren{\'e}e and H{\"o}nig, Wolfgang and Juckeland, Guido and Debus, Alexander and Kluge, Thomas and Schramm, Ulrich and Cowan, Tomas E and Sauerbrey, Roland and Bussmann, Michael},
  journal={Plasma Science, IEEE Transactions on},
  volume={38},
  number={10},
  pages={2831--2839},
  year={2010},
  publisher={IEEE}
}

@article{kong2011particle,
  title={Particle-in-cell simulations with charge-conserving current deposition on graphic processing units},
  author={Kong, Xianglong and Huang, Michael C and Ren, Chuang and Decyk, Viktor K},
  journal={Journal of Computational Physics},
  volume={230},
  number={4},
  pages={1676--1685},
  year={2011},
  publisher={Elsevier}
}

@article{dawson2008high,
  title={High-Performance Computing and Plasma Physics},
  author={Dawson, John M and Decyk, Viktor and Sydora, Richard and Liewer, Paulett},
  journal={Physics Today},
  volume={46},
  number={3},
  pages={64--70},
  year={2008},
  publisher={American Institute of Physics}
}

@article{abreu2011pic,
  title={PIC codes in new processors: A full relativistic PIC code in CUDA-enabled hardware with direct visualization},
  author={Abreu, Paulo and Fonseca, Ricardo and Pereira, Jo{\~a}o M and Silva, Lu{\'\i}s O and others},
  journal={Plasma Science, IEEE Transactions on},
  volume={39},
  number={2},
  pages={675--685},
  year={2011},
  publisher={IEEE}
}

@article{decyk2007upic,
  title={UPIC: A framework for massively parallel particle-in-cell codes},
  author={Decyk, Viktor K},
  journal={Computer Physics Communications},
  volume={177},
  number={1},
  pages={95--97},
  year={2007},
  publisher={Elsevier}
}

@article{decyk2011adaptable,
  title={Adaptable particle-in-cell algorithms for graphical processing units},
  author={Decyk, Viktor K and Singh, Tajendra V},
  journal={Computer Physics Communications},
  volume={182},
  number={3},
  pages={641--648},
  year={2011},
  publisher={Elsevier}
}

@article{horowitz1989qn3d,
  title={QN3D: A three-dimensional quasi-neutral hybrid particle-in-cell code with applications to the tilt mode instability in field reversed configurations},
  author={Horowitz, Eric J and Shumaker, Dan E and Anderson, David V},
  journal={Journal of Computational physics},
  volume={84},
  number={2},
  pages={279--310},
  year={1989},
  publisher={Elsevier}
}

@article{jolliet2007global,
  title={A global collisionless PIC code in magnetic coordinates},
  author={Jolliet, S and Bottino, Alberto and Angelino, P and Hatzky, Roman and Tran, TM and McMillan, BF and Sauter, O and Appert, K and Idomura, Yasuhiro and Villard, Laurent},
  journal={Computer Physics Communications},
  volume={177},
  number={5},
  pages={409--425},
  year={2007},
  publisher={Elsevier}
}

@article{tran1998global,
  title={Global gyrokinetic simulation of ion-temperature-gradient-driven instabilities using particles},
  author={Tran, Track M and Appert, K and Fivaz, M and Jost, G and Vaclavik, J and Villard, L},
  journal={Theory of fusion plasmas: in: J.W. Connor, E. Sindoni, J. Vaclavik (Eds.), Proceedings of the Joint Varenna-Lausanne International Workshop},
  pages={45--58},
  year={1998}
}

@inproceedings{ethier2005gyrokinetic,
  title={Gyrokinetic particle-in-cell simulations of plasma microturbulence on advanced computing platforms},
  author={Ethier, S and Tang, WM and Lin, Z},
  booktitle={Journal of Physics: Conference Series},
  volume={16},
  number={1},
  pages={1},
  year={2005},
  organization={IOP Publishing}
}
